On completeness of reducibility candidates as a semantics of strong normalization

This paper defines a sound and complete semantic criterion, based on reducibility candidates, for strong normalization of theories expressed in minimal deduction modulo \`a la Curry. The use of Curry-style proof-terms allows to build this criterion on the classic notion of pre-Heyting algebras and makes that criterion concern all theories expressed in minimal deduction modulo. Compared to using Church-style proof-terms, this method provides both a simpler definition of the criterion and a simpler proof of its completeness.

==> crcalach.tex <==
\newpage
\section{Complete reducibility candidates \`a la Church}

\subsection{About the (CR$_3$) property}

	\subsubsection{Context} We have detailed in the previous chapter the main method for proving strong normalization in different logical frameworks, using the set of so-called reducibility candidates. This method has been adapted for the logical framework of deduction modulo by defining the notion of pre-model, which is a set of reducibility candidates such that two equivalent propositions are interpreted by the same set. Then we have seen how this technique can be viewed as the building of a model on some sort of algebras called truth values algebras. And we have exhibited the particular truth values algebras of reducibility candidates $\calC$, concluding that having a $\calC$-valued model is a sound semantics for strong normalization in (minimal) deduction modulo. 
	
	\subsubsection{Contributions} The aim of this chapter is to analyse how  we can refine this notion of reducibility candidates in order to provide a sound and also complete semantics for strong normalization. We focus in this chapter on the logical framework of minimal deduction modulo. We define a refinement of truth values algebras (\tva\hspace{-1ex}), called language-dependent truth values algebras (\ldtva\hspace{-1ex}). We call them {\em language-dependent} since this new notion of algebra depends on the sets of closed terms of the sorts of the predicate language on which we build a theory in minimal deduction modulo. Then we exhibit two of these languages-dependent truth valuas algebras such that both provide a sound and complete semantics for strong normalization via models valued in them. The method for proving completeness uses a specificity of the first \ldtva we define: the fact that we consider only proofs of a proposition in its interpretation. We therefore define, given a theory \lang$_\equiv$, the \ldtva of $\equiv$-well-typed reducibility candidates. It allows us to capture exactly the proofs of a proposition, via sets of proof-terms which satisfy analog properties as the well-known ones of reducibility candidates. We then define a more general \ldtva $\cprime$ which is independent of the congruence relation $\equiv$ of the theory we consider . This \ldtva provides a general sound and complete semantics for strong normalization for all theories expressed in minimal deduction modulo (based on a same predicate language).
	%  While the first language-dependent truth values algebra we define

	
	\subsubsection{Outline} As a first step, we  analyze precisely the role of the (CR$_3$) property of reducibility candidates, and of the interpretation of the universal quantifier in the \tva of reducibility candidates, in proofs of strong normalization. This analysis suggests that both are responsible of the difficulties involved when trying to prove that having a model valued in reducibility candidates is a complete semantics for strong normalization, when trying to prove the converse of the adequacy lemma for that purpose. We first adapt the latter by defining language dependent truth values algebras which provide a functional interpretation of the universal quantifier, and then propose two adaptations of the (CR$_3$) property which define two new definitions of reducibility candidates as some particular \ldtvas. While the first depends on typing and therefore on the congruence relation which defines the theory we consider, the second one is theory-independent. We prove models valued in both these \ldtvas provide two different sound and complete semantics for strong normalization in minimal deduction modulo. Completeness of models valued in the second one is entailed by completeness  of models valued in the first one, by building a morphism of \ldtvas from the first one to the second one, inducing a mapping from models valued in the first one to models valued in the second one.
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bigskip
	\section{Are usual reducibility candidates complete ?}
	\label{aurdc}
		We saw, in the previous chapter that reducibility candidates are sound for strong normalization, in the sense that if we can build a set of reducibility candidates adapted to a logical framework then this logical framework is strongly normalizing. From a $\textsc{tva}$ point of view it means that having a $\calC$-valued model is a sufficient condition for a theory to be strongly normalizing in minimal deduction modulo. Then we may wonder whether reducibility candidates also are complete, i.e. whether having a $\calC$-valued model is also a necessary condition for a theory to be strongly normalizing. 
		
		In 1929, Gödel proved his completeness theorem concerning consistency of theories expressed in natural deduction. Gödel proved in \cite{Godel} that besides being a sound semantics, having a $\{0,1\}$-valued model is a complete semantics for the property of consistency of theories expressed in first order logic. In other words, he exhibited a correspondence, in first order logic, between truth an provability, between model theory and proof theory.
		Other completeness theorems have been proved: for higher order logic by Henkin \cite{Henkin} and for modal logic, by Kripke \cite{Kripke}. They both concern sound and complete semantics for consistency.
		
		As we saw in \ref{cean}, when we express theories in minimal deduction modulo, only within the congruence relation and not with axioms, the strong normalization of the theory we consider entails its cut elimination and therefore its consistency. Hence strong normalization implies consistency. The converse is not true, since there exists theories which have the cut elimination property, but which do not strongly normalize \cite{HermantThese}. Hence strong normalization is a strictly more powerful property than consistency. In this way, we can see the work presented in this section, as the natural following of the previous completeness theorems cited above.
		
		As we said in \ref{arc}, the main point of proofs of normalization using reducibility candidates is the adequacy lemma, which states that each proof-term which is a proof of a proposition belongs to the reducibility candidate associated to this proposition, and is therefore strongly normalizing. The first naïve idea to prove completeness of ${\cal C}$-valued models for strong normalization is to try to prove the converse of the adequacy lemma: each reducibility candidate associated to a proposition contains only proofs of this proposition, in order to obtain what we shall call {\em well-typed reducibility candidates}. We shall see, in the following that it is not possible with usual reducibility candidates, because of the definition of the interpretation of the universal quantifier in \tvas, and because of the (CR$_3$) property. We will therefore propose a new definition of algebras, and a modified version of the (CR$_3$) property in order to be able to prove the converse of the adequacy lemma.
		
		
	%	$$~$$
%		This follows the work of Gödel in [bib]: he proved that having a $\{0,1\}$-valued model is a complete condition for a theory to be consistent in predicate calculus. As we saw previously, strong normalization of a theory entails its cut elimination and therefore its consistency.
%		\\ bla bla 
%		\\ Introduire idée naïve : renverser l'adequacy lemma -> parler de well-typed red cand
%		\\ introduire (CR$_3$) et forall
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\medskip
		\subsection{About the (CR$_3$) property}
		\label{atcr3p}
			Let us first analyze the role of the (CR$_3$) property in soundness of reducibility candidates. As we can notice in chapter \ref{pnaamtn}, this property is used twice in proofs of normalization. First to prove that $\calC$-models are non empty since they contain all proof-variables, and moreover, all neutral normal proof-terms. And in a second step, to prove that abstractions of type $A \Ra B$ are in the interpretation of $A \Ra B$. We first recall the definition of (CR$_3$): we say that a set $E$ of proof-terms satisfies (CR$_3$) if and only if all neutral proof-terms whose all $\beta$-reducts are in $E$, are also in $E$.
			
			\subsubsection{Variables} As soon as a set of proof-terms satisfies (CR$_3$), it contains all neutral normal proof-terms, since they have no reduct. Therefore all reducibility candidates contain all neutral normal proof-terms, and, in particular, all proof-variables. We shall see in \ref{tponnpt} that this is one of the reasons why we cannot prove the converse of the adequacy lemma with usual reducibility candidates.
				
			\subsubsection{Abstractions} In order to prove that an abstraction $\lambda\alpha.\pi$ of type $A \Ra B$ is in the interpretation of $A \Ra B$, the method is to prove that for all elements $\pi'$ of the interpretation of $A$, $(\lambda \alpha.\pi)\pi'$ is in the interpretation of $B$, as you can notice in \ref{arc}. The main argument is that $(\lambda \alpha.\pi)\pi'$ is neutral and all its reducts are in the interpretation of $B$ (by induction hypothesis). We can notice that in this case, $(\lambda \alpha.\pi)\pi'$ is well-typed (of type $B$ namely) and non-normal. Those facts will be useful when we shall modify the (CR$_3$) property in the following.  
			
		\medskip
		
		Those two properties are essential in the proof of the adequacy lemma. We shall have to verify that the new definitions of reducibility candidates we shall propose in the following, still satisfy those properties, in order to prove that they are still sound for strong normalization.
			
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\medskip
		\subsection{The problem of neutral normal proof-terms}
		\label{tponnpt}
			The usual (CR$_3$) property prevents from proving the converse of the adequacy lemma: reducibility candidates do not contain only well-typed proof-terms. We say that they are {\em not adapted to typing}. In fact, all reducibility candidates contain all neutral normal proof-terms: as we have seen for variables, those proof-terms are neutral and do not have $\beta$-reducts. In particular, if $\alpha$ is a proof-variable, the proof-term $\alpha\alpha$ belongs to all reducibility candidates, and yet it cannot be well-typed in a strongly normalizing theory. Indeed, if there exists a context $\Gamma$ and a proposition $A$ such that $\Gamma \vdash \alpha \alpha : A$, then there exists propositions $B$ and $C$ such that $\Gamma \vdash \alpha : B$ and $\Gamma \vdash \alpha : B \Ra A$, by case analysis on the last rule used in the derivation of $\Gamma \vdash \alpha \alpha : A$. Hence we also have $B \equiv \equiv B \Ra A$. If we write $\delta = \lambda \alpha. \alpha \alpha$, we can then obtain $\Gamma \vdash \delta : B \Ra A$, since $\Gamma \vdash \alpha : B$ and $\Gamma \vdash \alpha \alpha : A$. Moreover, since $B \Ra A \equiv B$, we also have  $\Gamma \vdash \delta : B$, and we obtain $\Gamma \vdash \delta \delta : A$. 
			
			
	\bigskip
	
	If we note $\Pi_0$ the following typing judgement:
	
	\begin{prooftree}
      \RightLabel{{\scriptsize axiom}}% {\tiny $B \equiv B \Ra A$}}
      \AxiomC{~}
      \UnaryInfC{$\Gamma, \alpha:B \vdash \alpha : B \Ra A $}

	\RightLabel{{\scriptsize axiom}}
      \AxiomC{~}
      \UnaryInfC{$\Gamma, \alpha:B \vdash \alpha : B$}

	\RightLabel{{\scriptsize $\Ra$-elim}}
      \BinaryInfC{$\Gamma, \alpha:B \vdash \alpha\alpha : A$}

	\RightLabel{{\scriptsize $\Ra$-intro}}
      \UnaryInfC{$\Gamma \vdash \lambda \alpha.\alpha\alpha :B \Ra A$}
	\end{prooftree}
	
	\bigskip
	and $\Pi_1$ this one:
	
	\begin{prooftree}
      \RightLabel{{\scriptsize axiom}}% {\tiny $B \equiv B \Ra A$}}
      \AxiomC{~}
      \UnaryInfC{$\Gamma, \alpha:B \vdash \alpha : B \Ra A $}

	\RightLabel{{\scriptsize axiom}}
      \AxiomC{~}
      \UnaryInfC{$\Gamma, \alpha:B \vdash \alpha : B$}

	\RightLabel{{\scriptsize $\Ra$-elim}}
      \BinaryInfC{$\Gamma, \alpha:B \vdash \alpha\alpha : A$}

	\RightLabel{{\scriptsize $\Ra$-intro}~~$B \equiv B \Ra A$}
      \UnaryInfC{$\Gamma \vdash \lambda \alpha.\alpha\alpha :B$}
	\end{prooftree}
	
	\bigskip
	
	then we obtain:
	
	
	\begin{prooftree}
	\RightLabel{~}
	\AxiomC{$\Pi_0$}
      \UnaryInfC{$\Gamma \vdash \lambda \alpha.\alpha\alpha :B \Ra A$}


	\RightLabel{~}
	\AxiomC{$\Pi_1$}
        \UnaryInfC{$\Gamma \vdash \lambda \alpha.\alpha\alpha :B$}


      \RightLabel{{\scriptsize $\Ra$-elim}}
      \BinaryInfC{$\Gamma \vdash (\lambda \alpha.\alpha\alpha)(\lambda \alpha.\alpha\alpha) : A$}

    \end{prooftree}
	
	\bigskip
	
			
			Finally, $\alpha \alpha$ cannot be well-typed in a strongly normalizing theory, otherwise $\delta \delta$ would be also well-typed, whereas it is not even weakly normalizing since the only $\beta$-reduct of $\delta \delta$ is itself.
			
			We therefore have to modify this (CR$_3$) property in order to obtain a definition of well-typed reducibility candidates, but we also have to modify the interpretation of the universal quantifier as we shall see in the next subsection.
			
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\medskip
		\subsection{How to interpret the universal quantifier}
		\label{htituq}
		In the usual Truth Values Algebra $\calC$ of reducibility candidates, the interpretation of the universal quantifier is  defined as an intersection of a set of sets of proof-terms:
		$$\hatfa ~ \calE = \cap ~\calE$$ %\{\pi \textrm{ such that for all }t\textrm{ of sort }T, ~\pi t \in \calE\}$$
		
		%We recall the fact that $\hatT$ denotes the set of closed terms of sort T. 
		\noindent For all propositions $A$, term-variables $x$ of sort $T$, and valuations \linebreak  $\varphi \in \calV(\forall x.A)$, the interpretation of $\forall x.A$ and the valuation $\varphi$ is obtained from all interpretations of $A$ with the different valuations $\varphi + \langle x,t \rangle$, for $t \in \hatT$:
		
		$$\begin{array}{lll}
		\dd{\forall x.A}_\varphi & =  & \hatfa \{ \dd{A}_{\varphi + \langle x,t \rangle }, ~t \in \hatT \} \\
		~ & = & \{ \pi \textrm{ such that for all terms } t_1 \textrm{ and }t_2 \in \hatT,~\pi t_1 \in \dd{A}_{\varphi+ \langle x,t_2 \rangle} \}
		\end{array}$$
		
		In the particular case where $\hatT$ is chosen as the set of closed terms of sort $T$, we can notice that this definition of $\hatfa$ is not adapted to the notion of typing, because of the fact that $t_1$ and $t_2$ are not synchronized. If \linebreak $\Gamma \vdash \pi : \forall x.A$, and $t_1$, $t_2$ are two diferent closed terms in $\hatT$, then we do not have necessarily $\Gamma \vdash \pi t_1 : (t_2/x)A$. For example, in arithmetic, if we consider the proposition $\forall x. ~1+x = x+1$, we can build a proof of this proposition which will, applied to a term $z$, use $(z-1)$ times the axiom $y + (t+1) = (y+t)+1$.  Of course, when we apply this proof to $2$, we do not obtain a proof of $3+1 = 1+3$.
		
%		$$EXAMPLE~~~(egalite~?)$$
		\medskip
		
		In order to make interpretation of the universal quantifier adapted to the notion of typing, we have therefore to modify the notion of Truth Values Algebras. In order to synchronize $t_1$ and $t_2$ in the previous definition, we have first to consider a different interpretation of the universal quantifier for each sort of the language, and, secondly, we have to provide a interpretation of the universal quantifier which takes in argument a function an not a set of sets, in order to define a dependent intersection: 
		$$\dd{\forall x.A}_\varphi = \{ \pi \textrm{ such that for all } t \in \hatT,~\pi t \in \dd{A}_{\varphi+ \langle x,t \rangle} \}$$
		We then adapt the notion of truth values algebras by defining {\em language-dependent truth values algebras}, which  use $\hatfa$ as a dependent intersection. Those \ldtvas depend on the language as we have to know the sets of closed terms $\hatT$, to define such a synchronized interpretation of the universal quantifier. 
		
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\bigskip
		\subsection{Language-dependent truth values algebras}
		\label{ldtva}
		We define in this subsection {\em language-dependent truth values algebras} (\ldtva), which differ from usual truth values algebras on two points. First, as we already said in  \ref{mdm} and \ref{tva}, we only consider theories in deduction modulo where axioms are expressed only within the congruence relation and not with axioms. Therefore we do not distinguish {\em positive} truth values in the domain of a \ldtva. 
		%$$BLA~BLA$$
		
		Secondly, we always choose $\hatT$ as the set of closed terms of sort $T$ and we define the interpretation of the universal quantifier $\hatfa$ as a function which maps to elements of the domain, not subsets of the domain anymore but functions from $\hatT$ to the domain. 
		%This leads to parametrize $\hatfa$ by the sort we consider. 
		We therefore define a family of interpretations of the universal quantifier $(\hatfa_T)_{T\in \bbT}$, which are indexed by the different sorts of the language \lang ~we consider and more precisely, and which depend on the sets of closed terms of each of these sorts.  We then have to define \ldtvas, given a language \lang, this is why we call them {\em language-dependent}. Notice that the definition of a \ldtva does not depend on the whole language \lang, but only on the set of closed terms of each sort in $\bbT$, hence it only depends on $\bbT$ and $\bbF$.  Notice, finally, that those interpretations $\hatfa_T$ cannot always be defined on the whole set of functions from $\hatT$ to the domain, but only on one of its  subsets. We then define, for all sorts $T$, $\hcalA_T$, which is the subset of the set of functions from $\hatT$ to the domain, on which $\hatfa_T$ is defined. This gives the following definition.  
		
		\newpage
		
		\begin{definition}[Language-dependent \tvas\hspace{-1ex}]
	\index{Language-dependent Truth Values Algebras} ~\\
 Let \lang~ be a many-sorted language in predicate
logic.
\\$\hatalg$ is a \textsc{ldtva} for \lang ~ if and only if:
\vspace{-0.1cm}
\begin{iteMize}{-}
	\item $\calB$ is a set (called the {\em domain}),
	\item $\hatra$ is a function from $\calB \times \calB$ to $\calB$, 
	\item for all sorts $T \in \bbT$, $\hcalA_T$ is a set of functions from $\hatT$ to $\calB$,	
	\item  for all sorts $T \in \bbT$,  $\hatfa_T$ is a function from $\hcalA_T$ to $\calB$.
\end{iteMize}
\end{definition}

\noindent Notice that we shall write $\calB$ both for denominating the \textsc{ldtva} $\calB$ and its domain.  


%\begin{remark}
%We can notice that $\hatfa$ is now defined as a function from functions from $\hatT$ to $\calB$, to $\calB$, and not anymore as a function from $\Pa{\calB}$ to $\calB$ as in \tvas. we shall see in definition \ref{models} how this idea (\cite{Plotkin}) allows us to define dependent intersection.
%\end{remark}

	\smallskip
	In \ldtvas, we define models in a different way than in \tvas: we do not define anymore interpretations of propositions from  interpretations of atomic propositions, using interpretations of connectives, and then call them models if and only if they are {\em adapted to the congruence} (all equivalent propositions have the same interpretation). As in our presentation of pre models of section \ref{pmfdm}, given a \ldtva ~$\calB$, we define interpretations of propositions simply as functions which map every ordered pair of a proposition $A$ and a valuation in $\calV(A)$ to an element of $\calB$.

\begin{definition}[Interpretations]
	\index{Interpretations!on Language-dependent Truth Values Algebras} 
We call {\em $\calB$-valued interpretations} those functions which map every ordered pair of a proposition 
			$A$ and a valuation in $\calV(A)$ to an element of the domain of a \textsc{ldtva} $\calB$.
\end{definition}

\begin{definition}
We say that an interpretation of propositions is {\em non empty} if and only if each interpretation of a proposition and a valuation in $\calV(A)$ is a non empty set.
\end{definition}


\smallskip
And then we distinguish two properties of those interpretations. First, we say that an interpretation is a {\em model} if it is {\em adapted to the connectives} (with this definition, all \tva-interpretations are models since they are built inductively from the interpretation of connectives). And then we say that such a model is a model of a theory \lang$_\equiv$ if and only if all $\equiv$-equivalent propositions have the same interpretation (we say that the interpretation is {\em adapted to the congruence}). With these new definitions, we are able to define interpretations of propositions adapted to the congruence, while not necessarily adapted to the connectives, what we could not do with the original definition of models valued in \tvas\hspace{-1ex}. We shall see in section \ref{wtrc} how this new technique has been useful in order to prove completeness of such models (even if a simpler proof has been exhibited later).
\newpage

\begin{definition}[Models]
\index{Models!valued in Language-dependent Truth Values Algebras}
\label{models}~\\
%Let\lang be a many-sorted language in predicate logic, 
%let $\equiv$ be a congruence relation on propositions of minimal deduction based on \lang,
Let \lang$_\equiv$ be a theory expressed in minimal deduction modulo and \linebreak $\calB = \hatalg$ be a \textsc{ldtva} for \lang.
\begin{enumerate}[(1)]
%	\item[-]  We call {\em $\calB$-valued interpretations} those functions which map every ordered pair of a proposition 
%			$A$ and a valuation in $\calV(A)$ to an element of $\calB$.
%	\smallskip
	\item[-]  A $\calB$-valued interpretation $\dd{.}_.$ is a {\em $\calB$-valued model} \mbox{ if and only if:}
	\begin{iteMize}{-}
		\smallskip
		\item[-]  for all $A, B \in \calP$ and $\varphi \in \calV(A \Ra B)$, ~$\dd{A \Ra B}_\varphi = \dd{A}_\varphi~\hatra~ \dd{B}_\varphi$
 		\smallskip
		\item[-]  for all $A \in \calP$, $x$ of sort $T$ and $\varphi \in \calV(\forall x.A)$ \mbox{such that $x \notin \textsc{dom}(\varphi)$,}
				\\~~ $(t \mapsto \dd{\forall x.A}_{\varphi+\langle x,t\rangle}) \in \hcalA_T$~~and~~$\dd{\forall x.A}_\varphi = \hatfa_T (t \mapsto \dd{A}_{\varphi+\langle x,t\rangle})$
		\smallskip
		\item[-]  for all $A \in \calP$, $x$ of sort $T$, $t \in \hatT$ and $\varphi \in \calV(\forall x.A)$ \mbox{such that $x \notin \textsc{dom}(\varphi)$,}
			 ~$\dd{(t/x)A}_\varphi = \dd{A}_{\varphi + \langle x,t \rangle}$.
	\end{iteMize}
	\smallskip
	\item[-]  A $\calB$-valued model $\dd{.}_.$ is a {\em model of the theory \lang$_\equiv$} if and only if:
		for all $A,A' \in \calP$, $\varphi \in \calV(A)$ and $\psi \in \calV(A')$, \\if ~$\varphi A \equiv \psi A'$, \mbox{then ~$\dd{A}_\varphi = \dd{A'}_\psi$}
	
\end{enumerate}
\end{definition}

\smallskip

\begin{remark}
The previous conditions can be reformulated as:  
	\begin{enumerate}[(1)]
		\item Interpretations of propositions have to be {\em adapted to the connectives} $\Ra$ and $\forall$ to be a model.
		\item Models have to be {\em adapted to the congruence} to be a model of the associated theory.
	\end{enumerate}
\end{remark}

